Semantic Preserving Generative Adversarial Models

We introduce generative adversarial models in which the discriminator is replaced by a calibrated (non-differentiable) classifier repeatedly enhanced by domain relevant features. The role of the classifier is to prove that the actual and generated data differ over a controlled semantic space. We demonstrate that such models have the ability to generate objects with strong guarantees on their properties in a wide range of domains. They require less data than ordinary GANs, provide natural stopping conditions, uncover important properties of the data, and enhance transfer learning. Our techniques can be combined with standard generative models. We demonstrate the usefulness of our approach by applying it to several unrelated domains: generating good locations for cellular antennae, molecule generation preserving key chemical properties, and generating and extrapolating lines from very few data points. Intriguing open problems are presented as well.

==> aaaiSuppelmentary.tex <==

\begin{figure*}[h]
    \includegraphics[width=0.4\textwidth,height=0.25\textwidth]{lines.png}
  \caption{Generation and extrapolation using only 16 training points}
  \label{fig:lines}
\end{figure*}
